Cascade versus Direct Speech Translation: Do the Differences Still Make a Difference?

Five years after the first published proofs of concept, direct approaches to speech translation (ST) are now competing with traditional cascade solutions. In light of this steady progress, can we claim that the performance gap between the two is closed? Starting from this question, we present a systematic comparison between state-of-the-art systems representative of the two paradigms. Focusing on three language directions (English-German/Italian/Spanish), we conduct automatic and manual evaluations, exploiting high-quality professional post-edits and annotations. Our multi-faceted analysis on one of the few publicly available ST benchmarks attests for the first time that: i) the gap between the two paradigms is now closed, and ii) the subtle differences observed in their behavior are not sufficient for humans neither to distinguish them nor to prefer one over the other.

==> AudioErr1.tex <==
%\subsection{\mn{Manual Analysis of Audio-related errors}}
%\subsection{\mn{Errors Related to Audio  Understanding}}
%Errors and Audio Understanding
%ST Errors and Audio Understanding
%\label{subsec:man-audio}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% NOTE PRECEDENTI %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The automatic analysis did not highlight any systems’ differences with respect to audio duration and speech rate.
%However, recent studies have suggested that direct systems might be able to exploit information in the audio signal to overcome limitations of the cascade, e.g. better infer proper subtitle segmentation \cite{karakanta-etal-2020-42} or speaker-dependent gender phenomena \cite{bentivogli-etal-2020-gender}. 
%However, it is possible that \mt{the different type of input} (unpunctuated text vs. audio), leads to different behaviours. We conduct a manual analysis which aims to investigate systems’ behaviour for two audio-related aspects.
%\mg{Another possible source of different behaviors is the \st{different} content the two architectures access when generating the translation.
%The MT model of a cascade system is fed with unpunctuated text that can contain ercognition errors, while direct solutions are provided with the richer information constituted by the audio signal.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% \NOTE PRECEDENTI %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The different way the two architectures handle the input audio may impact differently the systems' ability to recognise speech. Our manual inspection of the systems' outputs led to two main groups of errors related to audio understanding:
We run a manual analysis of systems' outputs to understand whether the different way to handle the input affects their ability to recognise speech. This led to isolating two main groups of errors:



%\mt{Another possible source of different behaviors is the content the two architectures access when generating the translation. In the cascade, the ASR transcribes the audio and the produced text is then fed into the MT. The transcription is unpunctuated and can contain recognition errors. Direct solutions are provided with the richer information constituted by the audio signal.}


%\noindent \textbf{Errors due to wrong understanding of audio.}
\paragraph{Errors due to wrong audio understanding.}
%Such errors occur because of the inability of the systems to correctly understand the speech in the audio signal.
%\mg{They are easy to identify for the cascade systems, as they blatantly appear in the ASR output, while their detection is less trivial for the direct solutions that do not clearly expose what the model recognized from the audio. However, recognition errors can also be identified in this scenario, as they lead to a translation with a meaning different from the source and corresponding to a phonetically close content, e.g. \textit{nice voice} internally represented as \textit{nice boys} and then translated as \textit{bei ragazzi}. In light of the above, for the sake of a fair comparison the annotators had access only to the audio, reference human transcription and systems' output translations both for cascade and direct models.}
%
%
%This type of errors is easy to identify for the cascade systems, as they are evident in the ASR output, but difficult to spot for the direct ones, which  do not clearly expose what the model recognized from the audio. 
This type of errors is easy to identify in the cascade systems' output, as they are evident in the ASR transcripts, but difficult to spot in the direct ones, whose internal representations are by far less accessible.
%However, recognition errors can also be identified in this scenario, as they lead to a translation with a meaning different from the source and corresponding to a phonetically close content, e.g. \textit{nice voice} internally represented as \textit{nice boys} and then translated as \textit{bei ragazzi}. In light of the above, for the sake of a fair comparison the annotators had access only to the audio, reference human transcription and systems' output translations both for cascade and direct models.
However, recognition errors can also be identified in this scenario, as they lead to a translation with a meaning different from the source and corresponding to a phonetically close content, e.g. \textit{nice voice} internally represented as \textit{nice boys} and then translated as \textit{bei ragazzi}. In light of the above, for the sake of a fair comparison the annotators had access only to the audio, reference human 
%transcription 
transcripts and systems' output translations both for cascade and direct models.
%%%%, e.g. \textit{nice voice} internally represented as \textit{nice boys} and then translated as \textit{bei ragazzi}.
%In order not to bias the analysis in favour of the direct system, since these errors appear in the ASR output of the cascade but are hard to spot in the direct, the annotators had access only to the audio, human transcription and MT outputs.
%\mg{They are easy to identify for the cascade systems, as they blatantly appear in the ASR output, while their detection is less trivial for the direct solutions that do not clearly expose what the model recognized from the audio. However, recognition errors can also be identified in this scenario, as they lead to a translation with a meaning different from the source and corresponding to a phonetically close content, e.g. \textit{nice voice} internally represented as \textit{nice boys} and then translated as \textit{bei ragazzi}. In light of the above, for the sake of a fair comparison the annotators had access only to the audio, reference human transcription and systems' output translations both for cascade and direct models.}
%\mg{They are easy to identify for the cascade systems, as they appear blatantly in the ASR output, while\st{, for the direct solutions,} their detection is less trivial \mt{for the direct solutions}. However, the annotators were able to recognize them even in this case, as the output translation has a meaning different from the source and \mt{the source of errors are those} \st{corresponds to} words that are phonetically close to the audio content, e.g. \textit{nice voice} \mt{internally represented as \textit{nice boys} and then}  translated as \textit{bei ragazzi} \st{(nice boys).}}
%\lb{this analysis is difficult to justify: cascade errors based on asr, but how can you recognize errors made by direct? clearly explain the criteria followed by linguists }
The human annotation performed on the PE-Set and reported in Table~\ref{tab:understanding} shows that audio understanding errors are extremely common for both systems and all language pairs and may be the main chink in the armour of ST systems. Despite this, both the number of errors and the number of sentences affected by such errors is significantly lower for the direct system, suggesting that the direct approach is more successful in correctly recognizing speech. We observed that this was the case especially for ``more difficult'' sentences, such as sentences with bad audio quality and overlapping or disfluent speech%, and for the translation of acronyms and named entities
. Examples are provided in Table~\ref{tab:audio-examples}. 
%\mg{FIRST WE STATE THAT DIRECT IS BETTER, THEN WE POINT TO EXAMPLES IN TABLE 4: SO, I EXPECT TO SEE THE DIRECT TO DO BETTER IN TABLE 4, WHILE THERE IS ONE EXAMPLE IN WHICH DIRECT IS BETTER, ONE IN WHICH CASCADE IS BETTER AND ONE WHEN THEY ARE BOTH WRONG. I THINK IT IS VERY CONFUSING.}


\begin{table}[h]
    \centering
    \small
    \begin{tabular}{l|c|c|c|c||c|c}\hline
         & both & C & D & Total & C_{sent} & D_{sent}  \\ \hline
        de & 51 & 96 & 52 & 199 & 218 & 151\\
        es & 82 & 108 & 66 & 256 & 213 & 127 \\
        it & 87 & 82 & 69 & 238 & 141 & 135\\ \hline
    \end{tabular}
 %   \caption{Audio understanding errors and number of sentences containing at least one such error for Cascade and Direct systems in the PE set.}
    \caption{Audio understanding errors and number of sentences in the PE set containing at least one such error for Cascade and Direct systems.}

    \label{tab:understanding}
\end{table}



\begin{table}[th!]
 \centering
 \small
 \tabcolsep2pt
\begin{tabular}{ll}
\hline
%  \textsc{audio}  &  The great ... geneticist, \textbf{T.G. Dobzhansky}, ...  \\
%  \textsc{c }      &  Il grande genetista ... \textbf{Tg dub Jansky}, ...\\
%  \textsc{d }  & Il grande genetista ... \textbf{T.G. Dodgensky}, ...  \\
%  \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \textsc{audio}  &  to the \textbf{er- euh} \textit{[disfluency]} Egyptian government  \\
 \textsc{c }      & der \textbf{eruptiven} \textit{[Eng. ``eruptive'']} Regierung ...\\ %Ägyptens  
 
 \textsc{d }  & an die Regierung Ägyptens\\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textsc{audio}  &   This is called the \textbf{EyeWriter}... \\
% \textsc{c}      &  Questo si chiama \textit{eyewriter}...\\
% \textsc{d}  &  Questo si chiama \textbf{``I Rider''}... \\
% \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textsc{audio}  & \textbf{While} chimpanzees are...\\
%  \textsc{c }      &  \textit{[-]} Los chimpancés están\\
%  \textsc{d}  &  \textbf{Bueno} \textit{[Eng. ``well'']}, los chimpancés están  \\
% \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \textsc{audio}  &  dominated by \textbf{big, scary} guys,...  \\
 \textsc{c }      &   dominados por \textit{grandes} tipos \textit{aterradores} \\
 \textsc{d}  &   dominados por los chicos de \textbf{Big Kerry}  \\
\hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textsc{audio}  &  I think, like \textbf{her},...  \\
  \textsc{c }      &  Penso che, come \textbf{qui} \textit{[Eng. ``here'']}, ...\\
 \textsc{d}  &  Penso che, come i \textbf{capelli} \textit{[Eng. ``hair'']},  ... \\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textsc{audio}  &  I think, like \textbf{her},...  \\
%  \textsc{c }      &  Ich denke, wie \textbf{hier} spielen wir  \textit{[Eng. ``here'']}, \\
%  \textsc{d}  &  Ich denke, wie \textbf{sie} spielen wir \textit{[Eng. ``her'']},  \\
% \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
    \caption{Examples of audio understanding errors.} 
    \label{tab:audio-examples}
\end{table}
%\textsc{src}  &  ...going on along a \textbf{busy road}.  \\
% \textsc{c }      &  ...laufen entlang einer \textbf{BZero}. \textit{[Eng. ``B zero'']}\\
% \textsc{d }  & ...entlang einer \textbf{B.C. Straße.} \textit{[Eng. B.C. road]} \\
 
%\paragraph{Ability to recognize sentence type}\mbox{}\\
\noindent \textbf{Ability to recognize sentence type.} Prosody is central to the full understanding of a spoken text and differs depending on whether a sentence is affirmative or interrogative. Prosody is encoded in the 2D information received by the direct system, while the MT of the cascade, receiving unpunctuated input, may 
%be 
fail to retrieve the correct sentence-final punctuation. 
However, we found that both systems managed to translate the interrogative sentences correctly in most cases (24 out of 31 for the cascade, 25 out of 31 for the direct). This finding does not conclude that prosodic information is not useful or exploited by the direct system, but could be attributed to the syntactic structure of English questions, which is explicit and does not rely solely on prosody (compared to languages like Italian).


==> AudioErr2.tex <==
%\subsection{\mn{Manual Analysis of Audio-related errors}}
%\subsection{\mn{Errors Related to Audio  Understanding}}
%Errors and Audio Understanding
%ST Errors and Audio Understanding
%\label{subsec:man-audio}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% NOTE PRECEDENTI %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The automatic analysis did not highlight any systems’ differences with respect to audio duration and speech rate.
%However, recent studies have suggested that direct systems might be able to exploit information in the audio signal to overcome limitations of the cascade, e.g. better infer proper subtitle segmentation \cite{karakanta-etal-2020-42} or speaker-dependent gender phenomena \cite{bentivogli-etal-2020-gender}. 
%However, it is possible that \mt{the different type of input} (unpunctuated text vs. audio), leads to different behaviours. We conduct a manual analysis which aims to investigate systems’ behaviour for two audio-related aspects.
%\mg{Another possible source of different behaviors is the \st{different} content the two architectures access when generating the translation.
%The MT model of a cascade system is fed with unpunctuated text that can contain ercognition errors, while direct solutions are provided with the richer information constituted by the audio signal.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% \NOTE PRECEDENTI %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%While audio duration and speech rate are not informative 
%As a complement to 
Handling the input audio differently, the two 
%ST
approaches have inherent strengths and weaknesses. In particular, though suffering from the well-known scarcity of  sizeable training corpora,  direct solutions come with the promise \cite{sperber-paulik-2020-speech} of: \textit{i)} higher robustness to error propagation, and \textit{ii)} reduced loss of speech information 
%(e.g. prosody -- \cite{sperber-paulik-2020-speech}).
(e.g. prosody).
%Is this promise fulfilled
%In light of this promise,  our qualitative analysis looks at systems' ability to recognise speech.
Our next qualitative analysis tries to delve into these 
%aspects.
aspects by looking at audio understanding and prosody issues.
%Our complementary qualitative analysis focuses on  two relevant aspects in ST: audio understanding (related to error propagation) and prosody (on which the direct has a potential edge on the cascade)

\paragraph{Audio understanding.} Errors due to wrong 
%understanding of the audio
audio understanding are easy to identify for cascade systems -- since they are evident in the intermediate ASR transcripts -- but harder to spot for direct systems, whose internal representations are by far less accessible.
%
%However, some recognition errors can also be identified in this case, as they lead to translations that 
In this case, %however, 
errors can still be identified %in clearly wrong translations of 
%homophones 
through mistranslations %expressions (word, phrases) 
which are phonetically similar
%close 
to parts of the input audio -- e.g. \textit{nice voice} internally represented as \textit{nice boys} and translated in Italian as \textit{bei ragazzi}. 
%Other examples are reported in 
To spot such errors, 
our annotators 
carefully inspected the PE-set by comparing  the audio, reference human transcripts and systems' output translations both for the cascade and direct models. Some interesting examples of the identified 
%issues
errors are reported in Table~\ref{tab:audio-examples}.

%%%%% (\ding{55}) (\ding{51})
\begin{table}[th!]
 \centering
 \small
 \tabcolsep2pt
\begin{tabular}{ll}
\hline
 \textsc{audio}  &  to the \textbf{er- euh} \textit{[disfluency]} Egyptian government  \\
 \textsc{c}      & der \textbf{eruptiven} \textit{[Eng. ``eruptive'']} Regierung ...\\ %Ägyptens  
 
 \textsc{d}  & an die Regierung Ägyptens\\
\hline
 \textsc{audio}  &  dominated by \textbf{big, scary} guys,...  \\
 \textsc{c}      &   dominados por \textit{grandes} tipos \textit{aterradores} \\
 \textsc{d}  &   dominados por los chicos de \textbf{Big Kerry}  \\
\hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textsc{audio}  &  I think, like \textbf{her},...  \\
  \textsc{c}      &  Penso che, come \textbf{qui} \textit{[Eng. ``here'']}, ...\\
 \textsc{d}  &  Penso che, come i \textbf{capelli} \textit{[Eng. ``hair'']},  ... \\
\hline
\end{tabular}
   % \caption{Examples of audio understanding errors.} 
       \caption{\mn{Audio understanding errors.}} 

    \label{tab:audio-examples}
\end{table}

As shown in Table~\ref{tab:understanding}, 
audio understanding errors are extremely common for both systems 
%and
in all language pairs. However, both the number of errors and the number of sentences 
%affected by such errors
they affect
is significantly lower for the direct
%system.
one. 
%, suggesting that the direct approach is more successful in correctly recognizing speech. 
We observed that this 
%was
is the case especially for ``more difficult'' sentences, such as sentences with poor audio quality and overlapping or disfluent speech.

Though far from being conclusive (we acknowledge that, due to the ``opacity'' of direct models, their error counts might be slightly underestimated) 
%, even if carefully analysed)
this analysis seems to 
%support BLA.
confirm 
the theoretical advantages of direct ST. 
%We leave to future works a more thorough investigation on this aspect, as it  
This finding advocates for more thorough future 
%investigations, related to neural networks' interpretability, targeting 
investigations
%, dealing with neural networks' interpretability,
on neural networks' interpretability, targeting
its empirical  verification on larger and diverse 
%data.
benchmarks.
%In light of this, we believe that a more thorough investigation on this aspect, which  would deal with the 
%difficulties related to  
%hard problem of neural networks' interpretability, is 


%that direct ST has theoretical advantages


\begin{table}[h]
    \centering
    \small
    \begin{tabular}{l|c|c|c|c||c|c}\hline
         & both & C & D & Total & C$_{sent}$ & D$_{sent}$  \\ \hline
        de & 51 & 96 & 52 & 199 & 218 & 151\\
        es & 82 & 108 & 66 & 256 & 213 & 127 \\
        it & 87 & 82 & 69 & 238 & 141 & 135\\ \hline
    \end{tabular}
 %   \caption{Audio understanding errors and number of sentences containing at least one such error for Cascade and Direct systems in the PE set.}
    %\caption{Audio understanding errors and number of sentences in the PE-set containing at least one such error for Cascade and Direct systems.}
    \caption{Audio understanding errors in the PE-set  and number of sentences containing at least one such error.}
    \label{tab:understanding}
\end{table}


%\paragraph{Ability to recognize sentence type}\mbox{}\\
%\noindent \textbf{Ability to recognize sentence type.} 
%%%% ALINA
%\noindent \textbf{Prosody.}
%Prosody is central to the full understanding of a spoken text and 
%%%%%affects its written rendition. 
%differs depending on whether a sentence is affirmative or interrogative. Prosody is encoded in the 2D information received by the direct system, while the MT of the cascade, receiving unpunctuated input, may fail to retrieve the correct sentence-final punctuation.  However, we found that both systems managed to translate the interrogative sentences correctly in most cases (24 out of 31 cascade, 25 out of 31 direct). This finding does not conclude that prosodic information is not useful or exploited by the direct system, but could be attributed to the syntactic structure of English questions, which is explicit and does not rely solely on prosody (compared to languages like Italian). In fact, after careful inspection we identified examples (Table~\ref{tab:prosody}) where access to the prosody aided in disambiguating and correctly rendering the source sentence by the direct system.
%%%% MN
\noindent \textbf{Prosody.}
%Prosody is central to 
%%%%the full understanding of a spoken text
%disambiguating utterances, as it reflects language elements and speakers' features that 
%%%% may not be 
%are not encoded by grammar 
%%%% or by 
%and vocabulary choice. While it is directly encoded by the direct system, it might be lost in the unpunctuated input received by the MT component of a cascade one.
Prosody is central to disambiguating utterances, as it reflects language elements 
%and speakers' features 
which 
%are not
may not be encoded by grammar and vocabulary choice. While it is directly encoded by the direct system, it %might be 
is lost in the unpunctuated input received by the MT component of a cascade. Besides few interrogative sentences, 
our annotators were able to isolate only a 
%small number
handful
of utterances 
%in the PE-Set 
whose prosodic markers resulted in different interpretations by the two models. 
%only a small number of utterances in the PE-Set involve relevant prosodic phenomena. 
%
Concerning  interrogatives, 
%our manual analysis revealed that both 
both systems 
managed to translate 
%the interrogative sentences 
them correctly in most cases (cascade: 24/31; direct: 25/31). This is not surprising given the syntactic structure of English questions, which is explicit and does not rely solely on prosody 
%(compared to languages like Italian)
(e.g. compared to Italian).
%Nevertheless, in all the other cases
%where access to the prosody was crucial to t
%In all the other cases, access to the prosody proved to be crucial in disambiguating and correctly rendering the utterance meaning.
%
In all other cases  (examples in Table~\ref{tab:prosody}), the direct models' higher sensitivity to prosody  
%gives
seems to give them an edge on cascades in disambiguating and correctly rendering the utterance meaning.
%
Also this finding calls for future inquiries
%to check the regularity of 
checking the regularity 
%of this subtle difference observed in their behaviour.
of these behavioural differences  on larger datasets.


%Also in this case, deeper inquiries on larger datasets would definitely help to check the regularity of this subtle difference observed in their behaviour.

%Prosody is central to the full understanding of a spoken text and differs depending on whether a sentence is affirmative or interrogative. Prosody is encoded in the 2D information received by the direct system, while the MT of the cascade, receiving unpunctuated input, may fail to retrieve the correct sentence-final punctuation.  However, we found that both systems managed to translate the interrogative sentences correctly in most cases (24 out of 31 cascade, 25 out of 31 direct). This finding does not conclude that prosodic information is not useful or exploited by the direct system, but could be attributed to the syntactic structure of English questions, which is explicit and does not rely solely on prosody (compared to languages like Italian). In fact, after careful inspection we identified examples (Table~\ref{tab:prosody}) where access to the prosody aided in disambiguating and correctly rendering the source sentence by the direct system.


%%%%% (\ding{55})...(\ding{51})
\begin{table}[h]

\small
\setlength\tabcolsep{1.3pt}
    \centering
    \begin{tabular}{ll}
    \hline
      src &  Photos like this: construction going on \\
      C& Foto come questa costruzione  %Fotos, wie diese Konstruktion  
      \scriptsize \textit{[Photos like this construction]} \\
      D& Foto come queste: costruzione  % Fotos wie dieses: Eine Baustelle 
      \scriptsize \textit{[Photos like these: construction]} \\ \hline
      src & nation states — governments doing the attacks \\
      C& Regierungen der Nationalstaaten  \scriptsize \textit{[governments of nation states]} \\
      D& Nationen, Regierungen  \scriptsize \textit{[nations, governments]} \\ \hline
      src & %helicopter, 
      like the one we saw before, moving \\
      C& como el que vimos antes de moverse  \scriptsize \textit{[before moving]}\\ %elicottero come quello che abbiamo visto prima di muoversi \\
      D& como el que hemos visto antes, moviéndose  \scriptsize \textit{[before, moving]}\\%elicottero, come quello che abbiamo visto prima, che si muove \\
      \hline
    \end{tabular}
    %\caption{Examples of sentences where prosody leads to different renderings for Cascade and Direct.}
        \caption{\mn{The two approaches dealing with prosody.}}

    \label{tab:prosody}
\end{table}

%\begin{table}[h]\hline
%\small
%    \centering
%    \begin{tabular}{ll}
%      src &  Photos like this: construction going on \\
%      C&  Fotos, wie diese Konstruktion  \\
%      & en: \textit{[, like this construction]} \\
%      D& Fotos wie dieses: Eine Baustelle  \\
%      & en: \textit{[, like this: a construction]} \\ \hline
%      src & nation states — governments doing the attacks \\
%      C& die Regierungen der Nationalstaaten, die... \\
%      D& Nationen, Regierungen, die... \\ \hline
%      src & %helicopter,       like the one we saw before, moving \\
%      C& %elicottero      come quello che abbiamo visto prima di muoversi \\
%      D& %elicottero, 
%      come quello che abbiamo visto prima, che si muove \\
%     
%    \end{tabular}
%    \caption{Examples of sentences where prosody leads to different renderings for Cascade and Direct.}
%    \label{tab:prosody}
%\end{table}

==> LingErr1.tex <==
\subsection{\mn{Automatic Analysis}}
\label{subsec:auto-errors}
% Although the overall performance is very similar, we aim to shed light on the peculiar characteristics of each approach. To this purpose, we apply the automatic error classification  procedure described above to investigate what are the linguistic phenomena that the two approaches are best able to handle. 

%To carry out error analysis we rely on a publicly available tool that proved able to provide useful insights on what linguistic phenomena are best modeled by \mn{MT} systems~\citep{Bentivogli2018}.
For this analysis, we rely on a publicly available tool used in a similar previous work by \citep{Bentivogli2018} to analyse  what linguistic phenomena are best modeled by MT 
%systems~\citep{Bentivogli2018}
systems.\footnote{Details of the tool are in the supplementary material.} %\footnote{The tool, downloadable from \url{wit3.fbk.eu/2016-02}, is a modified version of the \textit{tercom} script  (\url{www.cs.umd.edu/~snover/tercom}) requiring the lemmatized versions of both systems' outputs and post-edits. To  lemmatize the data we used the \textit{TreeTagger} (\url{www.cis.uni-muenchen.de/~schmid/tools/TreeTagger}).} 
The tool exploits manual post-edits as well as HTER-based computations to detect and classify translation errors according to the main linguistic categories of lexicon, morphology and word order.  
%
%coarse-grained linguistic error classification
%
% Then, we focus on differences among MT systems
% with respect to morphology, lexical, and word order errors
%
% We automatically detect and classify translation errors, exploiting the methodology and tools used in~\citep{Bentivogli2018}.\footnote{The modified \textit{tercom} version created to support error annotation is available at \url{XXXX}} 
% The automatic procedure is based on HTER computation under the assumption that, since the post-edit is generated by correcting the ST output, it directly points to translation errors.
%
%\footnote{The modified \textit{tercom} version created to support error annotation is available at \url{XXXX}} 
%
% Translation error analysis, as a way to identify systems’ weaknesses and define priorities for their
% improvement, has received a fair amount of attention in the MT community. In this work we opt for the automatic detection and classification of translation errors based on manual post-edits of the MT output
%
%For the three language directions addressed in this study, 
Table~\ref{tab:allErrors} presents the distribution of 
%error 
the three categories for each approach.

As expected from HTER scores (see Table~\ref{tab:overall}), results vary across the language pairs. For en-it, systems show pretty much the same number of errors, with a percentage gain in favour of the cascade approach of only 1.1. For the other two pairs the differences are more marked, with an overall error reduction for the direct system for en-es (-6.71) and in favour of the cascade system for en-de (+6.72). 

% \begin{table*}[!h]
%     %\tabcolsep3pt
%     \centering 
%     \small
%     \begin{tabular}{l|r|r|r||r|r|r||r|r|r}
%     %\hline
%       & \multicolumn{3}{|c|}{en-it} & \multicolumn{3}{|c|}{en-es} & \multicolumn{3}{|c}{en-de}\\
%       \hline
%      & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$  \\
%     \hline
%     Lexical           &  2264       & 2264   & 0.00  & 2674 &	2497 &	-6.62  & 2481    & 2560   & +3.18\\
%     Morphology        &  382        &  416   & +8.90  & 431  &	416 &	-3.48  &  372     & 409    & +9.95\\
%     Reordering        &  179        & 172    & -3.91   & 204	 & 212	& +3.92  &  302   & 349  & +15.56 \\
%     Morph+Reord       &  51         &  54    & +5.88 & 104	 & 78	& -25.00 & 96   &  127     & +32.29  \\
 
%     \hline
%     Total                 & 2876   & 2906  & +1.04   &  3413 &	3203 &	-6.15   & 3251   & 3445  & +5.97\\
%     \hline 
%     % \hline
%     % Morphology (all)      &  337 &  14.60 & 368  & 16.08  & +9.20\\
%     % Reordering (all)      & 185  & 8.01  & 181  & 7.91  & -2.16\\
%     %\hline
%     \end{tabular}
%     \caption{Distribution of error types for both ST approaches. The absolute number of errors (\#) is presented together with the percentage error reduction/increase of the  direct system with respect to the cascade one ({$\Delta \%$}). The morphology+reordering category includes those cases where both a morphological and reordering error occur on the same word.
%     } 
%     \label{tab:allErrors}
% \end{table*}


\COMMENT{
% VERSIONE TABELLA DEL 27/01/2021
\begin{table*}[!h]
    %\tabcolsep3pt
    \centering 
    \small
    \begin{tabular}{l|r|r|r||r|r|r||r|r|r}
    %\hline
       & \multicolumn{3}{|c|}{en-de} & \multicolumn{3}{|c|}{en-es} & \multicolumn{3}{|c}{en-it}\\
       \hline
     & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$  \\
    \hline
    Lexical           & 2481    & 2560   & +3.18 &   2674 &	2497 &	-6.62  & 2264       & 2264   & 0.00  \\
    Morphology         & 468 &	536 &	+14.53 &   535  &	494 &	-7.66  & 433        &  470  & +8.55 \\
    Reordering        & 398	& 476 &	+19.60  & 308	 & 290	& -5.84  &  230        & 226    & -1.74   \\
 %   Morph+Reord       &  51         &  54    & +5.88 & 104	 & 78	& -25.00 & 96   &  127     & +32.29  \\
 
    \hline
    Total                  & 3347	& 3572	& +6.72     &  3517 &	3281 &	-6.71 & 2927   & 2960  & +1.13\\
 
 
    \hline 
    % \hline
    % Morphology (all)      &  337 &  14.60 & 368  & 16.08  & +9.20\\
    % Reordering (all)      & 185  & 8.01  & 181  & 7.91  & -2.16\\
    %\hline
    \end{tabular}
    \caption{Distribution of error types for both ST approaches. The absolute number of errors (\#) is presented together with the percentage error reduction/increase of the  direct system with respect to the cascade one ({$\Delta \%$}). The morphology+reordering category includes those cases where both a morphological and reordering error occur on the same word.
    } 
    \label{tab:allErrors}
\end{table*}
}

\begin{table}[!t]
    \tabcolsep2pt
    \centering 
    \footnotesize
    \begin{tabular}{l||r|r|r||r|r|r||r|r|r}
    %\hline
       & \multicolumn{3}{c||}{en-de} & \multicolumn{3}{c||}{en-es} & \multicolumn{3}{c}{en-it}\\
       \cline{2-10}
     & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{D} & $\Delta \%$ & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{D} & $\Delta \%$ & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{D} & $\Delta \%$ \\
    \hline
    L         & 2481    & 2560   & +3.2     & 2674 &	2497 &	-6.6 &  2264       & 2264   & 0.0\\
    M        & 468 &	536 &	+14.5 &  535  &	494 &	-7.7  &  433        &  470  & +8.6  \\
    R       & 398	& 476 &	+19.6  &   308	 & 290	& -5.8  &  230        & 226    & -1.7   \\
 %   Morph+Reord       &  51         &  54    & +5.88 & 104	 & 78	& -25.00 & 96   &  127     & +32.29  \\
 
    \hline
                     & 3347	& 3572	& +6.7    &  3517 &	3281 &	-6.7  & 2927   & 2960  & +1.1 \\
    \hline 
        \end{tabular}
    \caption{Distribution of Lexical, Morphological and Reordering 
    %errors for both ST approaches. 
    errors. 
    Absolute numbers are presented together with the percentage of reduction/increase of the  Direct system with respect to the Cascade one ({$\Delta \%$}). 
    } 
    \label{tab:allErrors}
\end{table}

%
%
%\mt{Looking at the behaviour of the two technologies, it is interesting to note that when the source and target languages are quite different both in morphology and in grammatical structure (\textit{i.e.} English and German), the cascade has less errors than the direct resulting in positive deltas (last column). When the two languages are quite similar in grammatical structure and the target language has a less complex morphology compared to German (i.e. English and Spanish) the direct results in less errors than the cascade in all the categories. In the case of English-Italian, ...  }
%
Looking at the distribution of errors across categories, while for en-es the direct system is always better and the percentage reduction is homogeneously distributed, for en-de the better performance of the cascade system is concentrated in the  morphology and word order categories. Since English and German are the most different languages in terms of morphology and word order, this result suggests that the cascade system has an edge over the direct in its ability to handle morphology and word reordering. \lb{This is further supported  by en-it, where the only difference between the two systems can be seen in the morphology category, in favour of the cascade system.}

%\mt{However, the morphological and reordering errors are in a significantly lower number compared to the lexical ones in all the language directions suggesting that their impact on the overall automatic metrics is marginal.  }



% PROF DI LINGUISTICA: Ci sono elementi che fanno pensare che possa essere meno ricco (i) plurale dei nomi in S quindi no differenza tra maschile e femminile, (ii) nei verbi non e' marcato mai il genere. PERO' lo spagnolo e' piu' avanti nella creazione di nomi femminili. 
% NON SI PUO' AFFERMARE CHE SIA MENO RICCO



%is slightly more inflected than Spanish, in particular in the verbal where the languages are similar to English-Spanish in term of structure of the sentences, but Italian communication marking more the gender and the verbal cases, the cascade is better in morphology, while the direct is better in reordering.  However, 



%has a marked morphology compared to Spanish (e.g. Italian marked more the gender and the verbal cases than Spanish), 

%the cascade is better in morphology, while the direct is better in reordering.  

%marche di genere e numero sui verbi


%\mt{To be changed from here} While this differences are similar, the distribution of the errors across the categories is quite different. Indeed, for en-es the lexical category shows a high error difference, whereas for en-de the impact of lexical errors is less noticeable and the highest difference in the number of errors is grouped into the morphology and word order categories.


%dalla distribuzione degli errori si vede che il direct patisce quando c'e' reordering e morfologia, mentre dov non reordering e morfologia vince il direct, sull'italiano invece che ha morfologia piu' ricca dello spagnolo, vince il cascadae, mentre avendo poco reordinering vince il direct. Alla fine anch se la morfologia e' meglio il cascade, pero' sono meno in numero per cui e' tutto ancora aperto.
%
% Considering each error category, lexical  errors represent  by  far  the  most  frequent  error category  for both approaches (79.26\%  and 77.97\%). 
%
% Furthermore, the error classification procedure provides information about the part-of-speech of each error, allowing for a deeper analysis. As for lexical errors, the direct system makes less errors than the cascade one especially on nouns and punctuation. As for morphology errors, the direct system makes more errors, especially on adjectives, verbs, and nouns.  For the other two categories, error increments/reductions are homogeneously distributed among word classes.

%\subsection{Fine-grained Lexical Error Analysis}
%\subsection{\mn{Manual Analysis of Lexical Errors}}
\subsection{\mn{Manual Analysis}}
\label{subsec:man-errors}

Since lexical  errors represent  by  far  the  most  frequent  error category  for both approaches and  all the language pairs addressed, we complemented the automatic analysis with a more fine-grained manual inspection, further distinguishing among lexical errors due to missing words, superfluous words, or incorrect lexical choice.\footnote{Various error taxonomies covering different levels of
granularity have been developed, and the distinction between these types of lexical errors is widely adopted, included the MQM$/$DQF standard   \url{http://www.qt21.eu/mqm-definition/definition-2015-06-16.html#dqf-mapping}}

%We decided to complement them with a manual error annotation of a subset of segments, to gain a better insight into the systems' outputs and understand if there are some specific features that differentiate them.  

The analysis was carried out on a subset of the PE set, created in such a way to be suitable for manual annotation: we removed sentences for which the output of the two systems was \textit{i)}  identical, \textit{ii)} judged correct by post-editors (HTER=0),
%and
\mg{or} \textit{iii)} \mg{not good enough to be reliably annotated for errors  (HTER$>$40\%).}
%lower than 40\%, since 
%%it is known that 
%outputs over that threshold are not good enough to be reliably annotated for errors.
The subsets resulted in 207 sentences for en-de,  238 for en-es, and  285 for en-it. 

This analysis revealed that, for all language pairs, wrong lexical choice is the most frequent type of error ($\sim$75\% of lexical errors on average) followed by missing words ($\sim$30\%), while superfluous words represent only $\sim$5\%.
Whereas errors due to lexical choice and superfluous words vary across languages, we observed a systematic behaviour with respect to missing words, i.e. words that are present in the audio but are not translated. As we can see in Table~\ref{tab:missing}, the direct systems lose more information from the source input than their cascade counterparts, in terms of both single words and entire sequences. 
It is particularly interesting to notice that also for en-es -- where the direct system is significantly stronger than the cascade -- the issue is still evident, although to a lesser extent.
Table~\ref{tab:examples} collects examples of the encountered lexical phenomena.

% Results in Table~\ref{tab:missing} show a systematic behaviour with respect to missing words, i.e. words that are present in the audio but are not translated: the direct systems loses more information from the source input than its cascade counterpart, in terms of both single words as well as entire sequences of words (numeri?).

% GROUPED           CASC    DIR     CASC    DIR     CASC    DIR
% Missing word	    53		83	||	26		40	||	25		34
% Missing phrase	14		18	||	10		11	||	6		10

% Missing words marked as DM in the mt-equal subset
% it 20 / 25
% es 6 / 7 
% en 5 / 8

\begin{table}[h]
    \centering
    \small
    \begin{tabular}{l||c|c||c|c||c|c|C}
    
    
    
    & \multicolumn{2}{c||}{single } & \multicolumn{2}{c||}{word }  & \multicolumn{3}{c}{total }\\
    & \multicolumn{2}{c||}{words } & \multicolumn{2}{c||}{sequences }  & \multicolumn{3}{c}{\# words}\\
       \cline{2-8}
            & C & D & C & D & C & D & $\Delta \%$   \\ \hline
        de  & 25 & 34 & 6  &  10 & 42 & 58 & +38.10\\
        es & 26  &  40 & 10  & 11   & 59 & 68 & +15.25\\
        it  & 53  &  83 &  14 & 18  & 96 & 128 & +33.33 \\ \hline
    \end{tabular}
    \caption{Missing words  for Cascade and Direct systems. Note that absolute numbers vary across languages as they reflect the different size of the annotated subsets.}
    \label{tab:missing}
\end{table}

% \begin{table}[h]
%     \centering
%     \small
%     \begin{tabular}{l|c|c|c}\hline
%          & C & D & $\Delta \%$   \\ \hline
%         de & 42 & 58 & +38.10\\
%         es & 59 & 68 & +15.25\\
%         it & 96 & 128 & +33.33 \\ \hline
%     \end{tabular}
%     \caption{Missing words  for Cascade and Direct systems in the PE set.}
%     \label{tab:missing}
% \end{table}

\begin{table}[th!]
 \centering
 \small
\begin{tabular}{ll}
\hline
\textsc{audio}  &  \textbf{Well} after two years, ...  \\
\textsc{c}      &  \textit{Bueno}, después de dos años, ... \\
\textsc{d} & \textbf{[ -- ]} Después de dos años, ...\\
\hline
\textsc{audio}  &  My wife \textbf{and kids} and I, moved to  ...  \\
\textsc{c}      &  Io e mia moglie \textit{e i miei figli} ci siamo trasferiti...\\
\textsc{d}  & Io e mia moglie \textbf{[ -- ]} ci siamo trasferiti...  \\
 \hline
%  \textsc{audio}  &  \textbf{Say, "Computer}, would you please make  ...  \\
% \textsc{c}      &  \textbf{[ -- ]} Por favor, ejecuten ...\\
% \textsc{d}  & \textit{Digamos, "Computadora}, ¿harías por favor  ...  \\
%  \hline
\textsc{audio}  &  ``That's fine'', \textbf{says} George,  \\
\textsc{c}      &  ``Das ist in Ordnung.'' \textbf{[ -- ]}  George,\\
\textsc{d}  & ``Das ist in Ordnung, \textbf{[ -- ]} George, \\
\hline
\end{tabular}
    \caption{Examples of missing words.} 
    \label{tab:examples}
\end{table}


 Finally, we  report that a non-negligible amount of missing words (ranging between 10\% and 20\%) is represented by \lb{discourse markers}, i.e. words or phrases used to connect and manage what is being said (e.g. ``you know'', ``well'', ``now''). Although this is a frequent phenomenon in speech, not translating discourse markers cannot be properly considered as an error, since markers \textit{i)} do not carry semantic information, and \textit{ii)} can be intentionally dropped in some use cases, such as subtitling. %interpreting.

% \begin{table}[h]
%     \centering
%     \small
%     \begin{tabular}{l|c|c|c|c|c}\hline
%          & both  & both  & C  & D  & Total  \\ 
%          &  dropped &  kept &  dropped & dropped  &   \\
%          \hline
%         it & 54  & 23  & 13  &  14 & 104\\
%         es & 20  & 62  &  11 & 17 & 110\\
%         de &  28 & 41  &  14 & 22 & 105\\ \hline
%     \end{tabular}
%     \caption{Discourse markers present in the PE set. for Cascade and Direct systems in the PE set.}
%     \label{tab:DM}
% \end{table}


% DISCOURSE MARKERS: all PE set analysed		
% IT systems manage DM in a completely opposite way: most of them are dropped and there are no differences between systems, while for ES and DE most of them are kept and the direct drops more than cascade.
% EN-IT
% both dropped	54
% both kept	23	|
% casc kept - dir dropped	14	
% casc dropped - dir  kept	13	
% TOT	104	

% EN-ES
% both dropped	20
% both kept	62
% casc kept - dir dropped	17
% casc dropped - dir  kept	11
% TOT	110

% EN-DE
% both dropped	28
% both kept	41
% casc kept - dir dropped	22
% casc dropped - dir  kept	14
% TOT	105



%MORPHOLOGY VA MEGLIO IL CASCADE ANCHE CON ANALISI MANUALE, IN PARTICOLARE RILEVATO PROBLEMA SUI VERBI




%Some observations are consistent across models and show some regularities:
%systems still have difficulties in the translation of proper names 

%En-de errors are related to a different capitalization of words (example 2). 
% Also, we are particularly interested in understanding whether the direct use of the audio signal has an effect on the translation of the direct approach. The manual inspection revealed that the direct output contains errors that can be attributed to audio processing problems, as in examples 3 and 4 (example 4 also shows a missing capitalization by the cascade system). 



==> LingErr2.tex <==
\subsection{\mn{Automatic Analysis}}
\label{subsec:auto-errors}

For this analysis, we rely on the publicly available tool\footnote{\url{wit3.fbk.eu/2016-02}} used  by \citet{Bentivogli2018} to analyse  what linguistic phenomena are best modeled by MT systems.
%\footnote{Details of the tool are in the supplementary material.} %\footnote{The tool, downloadable from \url{wit3.fbk.eu/2016-02}, is a modified version of the \textit{tercom} script  (\url{www.cs.umd.edu/~snover/tercom}) requiring the lemmatized versions of both systems' outputs and post-edits. To  lemmatize the data we used the \textit{TreeTagger} (\url{www.cis.uni-muenchen.de/~schmid/tools/TreeTagger}).} 
The tool exploits manual post-edits 
%
%
%
%as well as HTER-based computations to detect and classify translation errors according to the main linguistic categories of lexicon, morphology and word order. Table~\ref{tab:allErrors} presents  the distribution of the three categories for each approach.
and HTER-based computations to detect and classify translation errors according to three linguistic categories: lexicon, morphology and word order. Table~\ref{tab:allErrors} presents their distribution for each approach.  
%
%
%
%
%coarse-grained linguistic error classification
%
% Then, we focus on differences among MT systems
% with respect to morphology, lexical, and word order errors
%
% We automatically detect and classify translation errors, exploiting the methodology and tools used in~\citep{Bentivogli2018}.\footnote{The modified \textit{tercom} version created to support error annotation is available at \url{XXXX}} 
% The automatic procedure is based on HTER computation under the assumption that, since the post-edit is generated by correcting the ST output, it directly points to translation errors.
%
%\footnote{The modified \textit{tercom} version created to support error annotation is available at \url{XXXX}} 
%
% Translation error analysis, as a way to identify systems’ weaknesses and define priorities for their
% improvement, has received a fair amount of attention in the MT community. In this work we opt for the automatic detection and classification of translation errors based on manual post-edits of the MT output
%
%For the three language directions addressed in this study, 


%
%As expected from HTER scores (see Table~\ref{tab:overall}), results vary across the language pairs. For en-it, systems show pretty much the same number of errors, with a percentage gain in favour of the cascade approach of only 1.1. For the other two pairs the differences are more marked, with an overall error reduction for the direct system for en-es (-6.71) and in favour of the cascade system for en-de (+6.72).
As expected from the HTER scores 
%reported 
in Table~\ref{tab:overall}, results vary across language pairs. On en-it, systems show pretty much the same number of errors, with a slight percentage gain (only 1.1) in favour of the cascade. For the other two pairs, differences are more marked and opposite, with an overall error reduction for the direct system  on en-es (-6.7)  and in favour of the cascade  on en-de (+6.7). 


% \begin{table*}[!h]
%     %\tabcolsep3pt
%     \centering 
%     \small
%     \begin{tabular}{l|r|r|r||r|r|r||r|r|r}
%     %\hline
%       & \multicolumn{3}{|c|}{en-it} & \multicolumn{3}{|c|}{en-es} & \multicolumn{3}{|c}{en-de}\\
%       \hline
%      & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$  \\
%     \hline
%     Lexical           &  2264       & 2264   & 0.00  & 2674 &	2497 &	-6.62  & 2481    & 2560   & +3.18\\
%     Morphology        &  382        &  416   & +8.90  & 431  &	416 &	-3.48  &  372     & 409    & +9.95\\
%     Reordering        &  179        & 172    & -3.91   & 204	 & 212	& +3.92  &  302   & 349  & +15.56 \\
%     Morph+Reord       &  51         &  54    & +5.88 & 104	 & 78	& -25.00 & 96   &  127     & +32.29  \\
 
%     \hline
%     Total                 & 2876   & 2906  & +1.04   &  3413 &	3203 &	-6.15   & 3251   & 3445  & +5.97\\
%     \hline 
%     % \hline
%     % Morphology (all)      &  337 &  14.60 & 368  & 16.08  & +9.20\\
%     % Reordering (all)      & 185  & 8.01  & 181  & 7.91  & -2.16\\
%     %\hline
%     \end{tabular}
%     \caption{Distribution of error types for both ST approaches. The absolute number of errors (\#) is presented together with the percentage error reduction/increase of the  direct system with respect to the cascade one ({$\Delta \%$}). The morphology+reordering category includes those cases where both a morphological and reordering error occur on the same word.
%     } 
%     \label{tab:allErrors}
% \end{table*}


\COMMENT{
% VERSIONE TABELLA DEL 27/01/2021
\begin{table*}[!h]
    %\tabcolsep3pt
    \centering 
    \small
    \begin{tabular}{l|r|r|r||r|r|r||r|r|r}
    %\hline
       & \multicolumn{3}{|c|}{en-de} & \multicolumn{3}{|c|}{en-es} & \multicolumn{3}{|c}{en-it}\\
       \hline
     & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$ & Cascade & Direct & $\Delta \%$  \\
    \hline
    Lexical           & 2481    & 2560   & +3.18 &   2674 &	2497 &	-6.62  & 2264       & 2264   & 0.00  \\
    Morphology         & 468 &	536 &	+14.53 &   535  &	494 &	-7.66  & 433        &  470  & +8.55 \\
    Reordering        & 398	& 476 &	+19.60  & 308	 & 290	& -5.84  &  230        & 226    & -1.74   \\
 %   Morph+Reord       &  51         &  54    & +5.88 & 104	 & 78	& -25.00 & 96   &  127     & +32.29  \\
 
    \hline
    Total                  & 3347	& 3572	& +6.72     &  3517 &	3281 &	-6.71 & 2927   & 2960  & +1.13\\
 
 
    \hline 
    % \hline
    % Morphology (all)      &  337 &  14.60 & 368  & 16.08  & +9.20\\
    % Reordering (all)      & 185  & 8.01  & 181  & 7.91  & -2.16\\
    %\hline
    \end{tabular}
    \caption{Distribution of error types for both ST approaches. The absolute number of errors (\#) is presented together with the percentage error reduction/increase of the  direct system with respect to the cascade one ({$\Delta \%$}). The morphology+reordering category includes those cases where both a morphological and reordering error occur on the same word.
    } 
    \label{tab:allErrors}
\end{table*}
}

\begin{table}[!t]
    \tabcolsep2pt
    \centering 
    \footnotesize
    \begin{tabular}{l||r|r|r||r|r|r||r|r|r}
    %\hline
       & \multicolumn{3}{c||}{en-de} & \multicolumn{3}{c||}{en-es} & \multicolumn{3}{c}{en-it}\\
       \cline{2-10}
     & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{D} & $\Delta \%$ & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{D} & $\Delta \%$ & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{D} & $\Delta \%$ \\
    \hline
    L         & 2481    & 2560   & +3.2     & 2674 &	2497 &	-6.6 &  2264       & 2264   & 0.0\\
    M        & 468 &	536 &	+14.5 &  535  &	494 &	-7.7  &  433        &  470  & +8.6  \\
    R       & 398	& 476 &	+19.6  &   308	 & 290	& -5.8  &  230        & 226    & -1.7   \\
 %   Morph+Reord       &  51         &  54    & +5.88 & 104	 & 78	& -25.00 & 96   &  127     & +32.29  \\
 
    \hline
                     & 3347	& 3572	& +6.7    &  3517 &	3281 &	-6.7  & 2927   & 2960  & +1.1 \\
    \hline 
        \end{tabular}
    \caption{Distribution of Lexical, Morphological and Reordering 
    %errors for both ST approaches. 
    errors. 
    Absolute numbers are presented together with the percentage of reduction/increase of the  Direct system with respect to the Cascade one ({$\Delta \%$}). 
    } 
    \label{tab:allErrors}
\end{table}

%
%
%\mt{Looking at the behaviour of the two technologies, it is interesting to note that when the source and target languages are quite different both in morphology and in grammatical structure (\textit{i.e.} English and German), the cascade has less errors than the direct resulting in positive deltas (last column). When the two languages are quite similar in grammatical structure and the target language has a less complex morphology compared to German (i.e. English and Spanish) the direct results in less errors than the cascade in all the categories. In the case of English-Italian, ...  }
%
Looking at 
the distribution of errors across categories, 
%\mn{error distribution across categories,}
while for en-es the direct system is always better and the percentage reduction is homogeneously distributed, for en-de the better performance of the cascade 
%system 
is concentrated in the  morphology and word order categories. 
Since English and German are the most different languages in terms of morphology and word order, this result suggests that 
%the cascade system has an edge over the direct \mn{one} in its ability to handle morphology and word reordering.
cascade systems still have an edge on the direct ones in their ability to handle morphology and word reordering.
%\mn{Since, among the three languages, English and German are the most distant ones in terms of morphology and word order, this suggests that the cascade system has an edge over the direct one in its ability to handle morphology and word reordering.} 
% This is further supported  by en-it, where the only difference between the two systems can be seen in the morphology category, in favour of the cascade system.
This is further supported  by 
%en-it, where 
en-it: the only difference,  in favour of the cascade, is 
indeed 
observed in the morphology category.



%\mt{However, the morphological and reordering errors are in a significantly lower number compared to the lexical ones in all the language directions suggesting that their impact on the overall automatic metrics is marginal.  }



% PROF DI LINGUISTICA: Ci sono elementi che fanno pensare che possa essere meno ricco (i) plurale dei nomi in S quindi no differenza tra maschile e femminile, (ii) nei verbi non e' marcato mai il genere. PERO' lo spagnolo e' piu' avanti nella creazione di nomi femminili. 
% NON SI PUO' AFFERMARE CHE SIA MENO RICCO



%is slightly more inflected than Spanish, in particular in the verbal where the languages are similar to English-Spanish in term of structure of the sentences, but Italian communication marking more the gender and the verbal cases, the cascade is better in morphology, while the direct is better in reordering.  However, 



%has a marked morphology compared to Spanish (e.g. Italian marked more the gender and the verbal cases than Spanish), 

%the cascade is better in morphology, while the direct is better in reordering.  

%marche di genere e numero sui verbi


%\mt{To be changed from here} While this differences are similar, the distribution of the errors across the categories is quite different. Indeed, for en-es the lexical category shows a high error difference, whereas for en-de the impact of lexical errors is less noticeable and the highest difference in the number of errors is grouped into the morphology and word order categories.


%dalla distribuzione degli errori si vede che il direct patisce quando c'e' reordering e morfologia, mentre dov non reordering e morfologia vince il direct, sull'italiano invece che ha morfologia piu' ricca dello spagnolo, vince il cascadae, mentre avendo poco reordinering vince il direct. Alla fine anch se la morfologia e' meglio il cascade, pero' sono meno in numero per cui e' tutto ancora aperto.
%
% Considering each error category, lexical  errors represent  by  far  the  most  frequent  error category  for both approaches (79.26\%  and 77.97\%). 
%
% Furthermore, the error classification procedure provides information about the part-of-speech of each error, allowing for a deeper analysis. As for lexical errors, the direct system makes less errors than the cascade one especially on nouns and punctuation. As for morphology errors, the direct system makes more errors, especially on adjectives, verbs, and nouns.  For the other two categories, error increments/reductions are homogeneously distributed among word classes.

%\subsection{Fine-grained Lexical Error Analysis}
%\subsection{\mn{Manual Analysis of Lexical Errors}}
\subsection{\mn{Manual Analysis}}
\label{subsec:man-errors}

Since lexical  errors represent
by  far  the  
%most  frequent  error category 
 most frequent category for both approaches
%and  all the language pairs addressed, we complemented
in  all language pairs, we complement
the automatic analysis with a more fine-grained manual inspection, further distinguishing among lexical errors
%\mn{those}
% \mn{those errors}
due to missing words, 
%superfluous words, or incorrect lexical choice
extra words, or wrong lexical choice.\footnote{Various error taxonomies covering different levels of
granularity have been developed, and the distinction between these types of lexical errors is widely adopted, included the 
%MQM/DQF standard \url{http://www.qt21.eu/mqm-definition/definition-2015-06-16.html#dqf-mapping}}
%\url{http://www.qt21.eu/quality-metrics/}}
DQF-MQM -- \url{https://info.taus.net/dqf-mqm-error-typology-templ}}
%
%We decided to complement them with a manual error annotation of a subset of segments, to gain a better insight into the systems' outputs and understand if there are some specific features that differentiate them.  

The analysis was
%\mn{is}
carried out on 
%a subset 
subsets
of the 
%PE set, created 
% \mn{PE-Set, isolated}
PE-set, created
in such a way to be suitable for manual annotation: we removed sentences for which the output of the two systems
%was
is:
\textit{i)}  identical, \textit{ii)} judged correct by post-editors (HTER=0),
%and
or \textit{iii)} 
%not good enough 
too poor
to be reliably 
annotated for errors  (HTER$>$40\%).
%\mn{error annotated (HTER$>$40\%).}
%lower than 40\%, since 
%%it is known that 
%outputs over that threshold are not good enough to be reliably annotated for errors.
%
%
%
%The subsets resulted 
The resulting data consist in 207 sentences for en-de,  238 for en-es, 
and  
285 for en-it. 

This analysis revealed that, for all language pairs, wrong lexical choice is the most frequent 
%type of error
error type
($\sim$75\% of lexical errors on average) followed by missing words ($\sim$30\%), 
%while  superfluous words represent only $\sim$5\%
%while extra words represent only $\sim$5\% of the cases.
and extra words ($\sim$5\%).

%Whereas
While
errors due to lexical choice and superfluous words vary across languages, we observed a systematic behaviour with respect to missing words
%, i.e. words that are present in the audio but are not translated.
(words that are present in the audio but are not translated). As we can see in Table~\ref{tab:missing}, 
%the 
direct systems lose more information from the source input than their cascade counterparts, in terms of both single words and 
%entire
contiguous word
sequences. 
It is particularly interesting to notice that also for en-es -- where the direct system is significantly stronger than the cascade -- the issue is still evident, although to a lesser extent.
Table~\ref{tab:examples} collects examples of the encountered lexical phenomena.

% Results in Table~\ref{tab:missing} show a systematic behaviour with respect to missing words, i.e. words that are present in the audio but are not translated: the direct systems loses more information from the source input than its cascade counterpart, in terms of both single words as well as entire sequences of words (numeri?).

% GROUPED           CASC    DIR     CASC    DIR     CASC    DIR
% Missing word	    53		83	||	26		40	||	25		34
% Missing phrase	14		18	||	10		11	||	6		10

% Missing words marked as DM in the mt-equal subset
% it 20 / 25
% es 6 / 7 
% en 5 / 8

\begin{table}[h]
    \centering
    \small
    \begin{tabular}{l||c|c||c|c||c|c|C}
    
    
    
    & \multicolumn{2}{c||}{single } & \multicolumn{2}{c||}{word }  & \multicolumn{3}{c}{total }\\
    & \multicolumn{2}{c||}{words } & \multicolumn{2}{c||}{sequences }  & \multicolumn{3}{c}{\# words}\\
       \cline{2-8}
            & C & D & C & D & C & D & $\Delta \%$   \\ \hline
        de  & 25 & 34 & 6  &  10 & 42 & 58 & +38.10\\
        es & 26  &  40 & 10  & 11   & 59 & 68 & +15.25\\
        it  & 53  &  83 &  14 & 18  & 96 & 128 & +33.33 \\ \hline
    \end{tabular}
    \caption{Missing words  for Cascade and Direct systems. Note that absolute numbers vary across languages as they reflect the different size of the annotated subsets.}
    \label{tab:missing}
\end{table}

% \begin{table}[h]
%     \centering
%     \small
%     \begin{tabular}{l|c|c|c}\hline
%          & C & D & $\Delta \%$   \\ \hline
%         de & 42 & 58 & +38.10\\
%         es & 59 & 68 & +15.25\\
%         it & 96 & 128 & +33.33 \\ \hline
%     \end{tabular}
%     \caption{Missing words  for Cascade and Direct systems in the PE set.}
%     \label{tab:missing}
% \end{table}

\begin{table}[th!]
 \centering
 \small
\begin{tabular}{ll}
\hline
\textsc{audio}  &  \textbf{Well} after two years, ...  \\
\textsc{c}      &  \textit{Bueno}, después de dos años, ... \\
\textsc{d} & \textbf{[ -- ]} Después de dos años, ...\\
\hline
\textsc{audio}  &  My wife \textbf{and kids} and I, moved to  ...  \\
\textsc{c}      &  Io e mia moglie \textit{e i miei figli} ci siamo trasferiti...\\
\textsc{d}  & Io e mia moglie \textbf{[ -- ]} ci siamo trasferiti...  \\
 \hline
%  \textsc{audio}  &  \textbf{Say, "Computer}, would you please make  ...  \\
% \textsc{c}      &  \textbf{[ -- ]} Por favor, ejecuten ...\\
% \textsc{d}  & \textit{Digamos, "Computadora}, ¿harías por favor  ...  \\
%  \hline
\textsc{audio}  &  ``That's fine'', \textbf{says} George,  \\
\textsc{c}      &  ``Das ist in Ordnung.'' \textbf{[ -- ]}  George,\\
\textsc{d}  & ``Das ist in Ordnung, \textbf{[ -- ]} George, \\
\hline
\end{tabular}
    \caption{Examples of missing words.} 
    \label{tab:examples}
\end{table}


 Finally, we  report that a non-negligible amount of missing words (ranging between 10\% and 20\%) is represented by discourse markers, i.e. words or phrases used to connect and manage what is being said (e.g. ``you know'', ``well'', ``now''). Although this is a frequent phenomenon in speech, not translating discourse markers cannot be properly considered as an error, since markers \textit{i)} do not carry semantic information, and \textit{ii)} can be intentionally dropped in some use cases, such as subtitling. 
 
 
 %interpreting.

% \begin{table}[h]
%     \centering
%     \small
%     \begin{tabular}{l|c|c|c|c|c}\hline
%          & both  & both  & C  & D  & Total  \\ 
%          &  dropped &  kept &  dropped & dropped  &   \\
%          \hline
%         it & 54  & 23  & 13  &  14 & 104\\
%         es & 20  & 62  &  11 & 17 & 110\\
%         de &  28 & 41  &  14 & 22 & 105\\ \hline
%     \end{tabular}
%     \caption{Discourse markers present in the PE set. for Cascade and Direct systems in the PE set.}
%     \label{tab:DM}
% \end{table}


% DISCOURSE MARKERS: all PE set analysed		
% IT systems manage DM in a completely opposite way: most of them are dropped and there are no differences between systems, while for ES and DE most of them are kept and the direct drops more than cascade.
% EN-IT
% both dropped	54
% both kept	23	|
% casc kept - dir dropped	14	
% casc dropped - dir  kept	13	
% TOT	104	

% EN-ES
% both dropped	20
% both kept	62
% casc kept - dir dropped	17
% casc dropped - dir  kept	11
% TOT	110

% EN-DE
% both dropped	28
% both kept	41
% casc kept - dir dropped	22
% casc dropped - dir  kept	14
% TOT	105



%MORPHOLOGY VA MEGLIO IL CASCADE ANCHE CON ANALISI MANUALE, IN PARTICOLARE RILEVATO PROBLEMA SUI VERBI




%Some observations are consistent across models and show some regularities:
%systems still have difficulties in the translation of proper names 

%En-de errors are related to a different capitalization of words (example 2). 
% Also, we are particularly interested in understanding whether the direct use of the audio signal has an effect on the translation of the direct approach. The manual inspection revealed that the direct output contains errors that can be attributed to audio processing problems, as in examples 3 and 4 (example 4 also shows a missing capitalization by the cascade system). 



==> eval1.tex <==
%%%%SCOMMENTARE SE SI RIPORTA NEL TEX
%\subsection{Evaluation Methodology}
%\label{ssec:method}











% The core of our multi-faceted evaluation is based on post-editing, which is one of the most prominent  methodologies  used  for translation quality  assessment~\citep{BentivogliIWSLT:2018}. 
% It was the focus of various studies \citep{Snover:06,Denkowski:2010,snover2009fluency,C16-1294} and was chosen as the official evaluation in large-scale shared tasks, such as IWSLT from 2013 to 2017~\citep{Cettolo:2013} and the MT Quality Estimation Task at WMT-2015~\citep{Bojar2015FindingsOT}.

The core of our multi-faceted evaluation is based on post-editing (PE). 
\lb{In PE-based evaluation, system outputs are post-edited, \textit{i.e.} manually corrected, \mt{according to the source language}. The original outputs are then evaluated against their post-edited versions through TER-based automatic metrics \cite{Snover:06}. 
The advantage of  relying on the post-edit as  reference translation is that only true errors in the system's output are counted, and not those differences due to linguistic variation, which are accounted for by post-editors.}

PE-based evaluation is one of the most prominent  methodologies  used  for translation quality  assessment~\citep{Snover:06,Denkowski:2010,snover2009fluency,C16-1294,BentivogliIWSLT:2018} and was chosen as  official evaluation in large-scale shared tasks, such as IWSLT from 2013 to 2017~\citep{Cettolo:2013} and the MT Quality Estimation Task at WMT-2015~\citep{Bojar2015FindingsOT}.
This offers us a consolidated framework and best practices on which we can draw upon in our experiments. 

The evaluation data used in this study is based on MuST-C~\citep{MuST-Cjournal}, which is the largest freely available multilingual corpus for ST. It comprises TED talks and covers 14 language directions, \lbf{with English audio segments automatically aligned with their corresponding manual transcriptions and translations.} The \textit{Common} en-de$/$es$/$it test sets contain the same 27 talks for around 2,500 largely overlapping segments,\footnote{MuST-C talks are automatically segmented and  aligned and can result in different segments across languages.} allowing for sound cross-language comparisons.

%The MuST-C \textit{Common} test set includes segments from talks that are common to all directions, thus making it possible to evaluate and compare systems across languages. 
 %The \textit{Common} test sets of the three directions addressed in this paper are composed of the same 27 TED talks, for a total of around 2,500 segments, and include one reference translation manually created from scratch. 
 
% For each language direction, we selected a subset of 550 segments -- henceforth \textit{PE-set} -- corresponding to about 10,000 English source words. To ensure the quality of the PE-set, we carried out a manual preparatory check and included only those segments i) containing speech and ii) for which  audio-transcript-translation alignment was correct. 

For each language direction, we selected the same English audio portions from each talk, so to obtain representative groups of consecutive segments which are comparable across languages.
Furthermore, to ensure the quality of the data, we carried out a manual preparatory check and included only those segments i) containing speech and ii) for which  audio-transcript-translation alignment was correct. The resulting test set -- henceforth \textit{PE-set} -- is composed of 550 segments, corresponding to about 10,000 English source words.

%%%%%%%%%%%%%%%%%%%%%%
% PROCEDURA SEGUITA
% Sentences were selected in a way to represent all the talks in the dataset proportionally to their length.  For each talk, three groups of consecutive sentences were selected from different parts of the talk: one close to the beginning, one in the middle, and one close to the end. The same selection criterion was applied to all the $11$ sections of MuST-C subject to manual evaluation, so to maximize the overlap between the sentences in the different languages and ensure results' comparability.
%%%%%%%%%%%%%%%%%%%%%%



%(around 90\%).
%
% For each language direction we selected a subset  of 550 segments -- henceforth \textit{PE-set} -- corresponding to about 10,000 English source words. These segments \textit{(i)} represent all the 27 common talks (groups of consecutive segments were extracted from different parts of each talk) and \textit{(ii)} were manually checked to ensure the correctness of the \textit{audio}-\textit{transcript}-\textit{translation} alignment, which in MuST-C is carried out automatically. 
%%Note that the PE-sets created for the three language pairs are not completely identical for two reasons: i) MuST-C talks are automatically segmented and  can thus result in different segments across languages; ii) we discarded all those segments for which  audio-transcript-translation alignment turned out to be incorrect (around 10\%). Although not exactly identical, the three PE-sets are largely overlapping.



Our cascade and direct systems (see $\S$\ref{ssec:systems}) were then run on the PE-sets to be post-edited according to the experimental procedure adopted in the IWSLT PE-based evaluations campaigns.
%~\citep{Cettolo:2013}. 
To guarantee high quality post-edits, we hired two professional translators with experience in  subtitling and post-editing. 
%%%%%AGGIUNTO PER RISPONDERE A MARCO
\lb{Furthermore, in order to cope with translators' variability (i.e. one translator could systematically correct more than the other), the outputs of the two ST systems were randomly assigned to them, ensuring that each translator worked on all the segments, equally post-editing both systems}
%
The post-editing task was run using a traditional CAT tool, which displays the manual transcript of the audio together with the ST output to be edited. However, since ST systems take as input an audio signal, we also provided translators with the audio file of each segment, and asked them to post-edit strictly according to it.\footnote{The \textit{ad-hoc} ST PE guidelines that were given to translators are included in the supplementary material.} 

The collected post-edits are exploited to assess overall systems' performance as well as to carry out (semi-)automatic analyses aimed to shed light on possible systematic differences between the two paradigms. These analyses are complemented by several fine-grained manual investigations \lb{aimed to explore specific aspects in the behaviours of the systems. These inspections are }carried out directly comparing the audio inputs with the systems' outputs, and do not require post-edits. 
Because of its linguistic nature, the annotation of the outputs was carried out by researchers with a strong background in linguistics and translation studies, and who have an excellent knowledge of both English and the target languages (C2 or native speaker).


==> eval2.tex <==
%%%%SCOMMENTARE SE SI RIPORTA NEL TEX
%\subsection{Evaluation Methodology}
%\label{ssec:method}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The core of our multi-faceted evaluation is based on post-editing (PE). 
% \lb{In PE-based evaluation, system outputs are post-edited, \textit{i.e.} manually corrected, \mt{according to the source language}. The original outputs are then evaluated against their post-edited versions through TER-based automatic metrics \cite{Snover:06}. 
% The advantage of  relying on the post-edit as  reference translation is that only true errors in the system's output are counted, and not those differences due to linguistic variation, which are accounted for by post-editors.}

%PE-based evaluation is one of the most prominent  methodologies  used  for translation quality  assessment~\citep{Snover:06,Denkowski:2010,snover2009fluency,C16-1294,BentivogliIWSLT:2018} and was chosen as  official evaluation in large-scale shared tasks, such as IWSLT from 2013 to 2017~\citep{Cettolo:2013} and the MT Quality Estimation Task at WMT-2015~\citep{Bojar2015FindingsOT}. This offers us a consolidated framework and best practices on which we can draw upon in our experiments. 

%For each language direction, we selected the same English audio portions from each talk, so to obtain representative groups of consecutive segments which are comparable across languages. Furthermore, to ensure the quality of the data, we carried out a manual preparatory check and included only those segments i) containing speech and ii) for which  audio-transcript-translation alignment was correct. The resulting test set -- henceforth \textit{PE-set} -- is composed of 550 segments, corresponding to about 10,000 English source words.

%%% PARTE SU MUSTC
%The evaluation data used in this study is based on MuST-C~\citep{MuST-Cjournal}, which is the largest freely available multilingual corpus for ST. It comprises TED talks and covers 14 language directions, with English audio segments automatically aligned with their corresponding manual transcriptions and translations. The \textit{Common} en-de$/$es$/$it test sets contain the same 27 talks for around 2,500 largely overlapping segments,\footnote{MuST-C talks are automatically segmented and  aligned and can result in different segments across languages.} allowing for sound cross-language comparisons.
%
%For each language direction, we selected the same English audio portions from each talk, so to obtain representative groups of consecutive segments which are comparable across languages. Furthermore, to ensure the quality of the data, we carried out a manual preparatory check and included only those segments i) containing speech and ii) for which  audio-transcript-translation alignment was correct. The resulting test set -- henceforth \textit{PE-set} -- is composed of 550 segments, corresponding to about 10,000 English source words.
%%%
%
% Our cascade and direct systems (see $\S$\ref{ssec:systems}) were then run on the PE-sets to be post-edited according to the experimental procedure adopted in the IWSLT PE-based evaluations campaigns.
% %~\citep{Cettolo:2013}. 
% To guarantee high quality post-edits, we hired two professional translators with experience in  subtitling and post-editing. 
% %%%%%AGGIUNTO PER RISPONDERE A MARCO
% \lb{Furthermore, in order to cope with translators' variability (i.e. one translator could systematically correct more than the other), the outputs of the two ST systems were randomly assigned to them, ensuring that each translator worked on all the segments, equally post-editing both systems}
% %
% The post-editing task was run using a traditional CAT tool, which displays the manual transcript of the audio together with the ST output to be edited. However, since ST systems take as input an audio signal, we also provided translators with the audio file of each segment, and asked them to post-edit strictly according to it.\footnote{The \textit{ad-hoc} ST PE guidelines that were given to translators are included in the supplementary material.} 

% The collected post-edits are exploited to assess overall systems' performance as well as to carry out (semi-)automatic analyses aimed to shed light on possible systematic differences between the two paradigms. These analyses are complemented by several fine-grained manual investigations \lb{aimed to explore specific aspects in the behaviours of the systems. These inspections are }carried out directly comparing the audio inputs with the systems' outputs, and do not require post-edits. 
% Because of its linguistic nature, the annotation of the outputs was carried out by researchers with a strong background in linguistics and translation studies, and who have an excellent knowledge of both English and the target languages (C2 or native speaker).




\paragraph{Data.}
Our evaluation data are drawn from the TED-based MuST-C corpus~\citep{MuST-Cjournal},  
the largest
%a large
freely available multilingual corpus for ST. It covers 14 language directions, with English audio segments automatically aligned with 
%their
the corresponding manual transcriptions and translations. The MuST-C \textit{Common} en--de/es/it test sets contain the same 27 talks for around 2,500 largely overlapping segments.\footnote{Note, however, that due to automatic segmentation and alignment of the talks, segments can vary across languages.}
For each language 
%direction,
pair,
we selected from MuST-C \textit{Common} the same English audio portions from each talk, so as to obtain representative groups of consecutive segments 
%which
that
are comparable across languages. Furthermore, to ensure
%the quality of the data,
high data quality, we carried out a 
%manual preparatory 
preliminary manual
check and included only those segments \textit{i)} containing only speech and \textit{ii)} for which  \textit{audio-transcript-translation} alignment is correct. For each language pair, the resulting test sets -- henceforth \textit{PE-sets} -- are composed of 550 segments, corresponding to about 10,000 English source words.
%\footnote{MuST-C talks are automatically segmented and  aligned and can result in different segments across languages} allowing for sound cross-language comparisons.



%\paragraph{Analysis based on post-edits.} 
\paragraph{Post-editing.} 

% A key ingredient of our multi-faceted analysis is human post-editing (PE), which consists in manually correcting system outputs according to the input (the source audio in our case). 
% %In PE-based evaluation, the collected post-edits are used as reference to evaluate the original outputs
% In PE-based evaluation, the original outputs are then 
% %evaluated through TER-based automatic metrics \cite{Snover:06} against their post-edited version used as reference.
% compared against their post-edited version to compute TER-based automatic metrics \cite{Snover:06}. This allows for counting only the true errors made by a system instead of 
% penalising also 
% %those differences due to linguistic variation with respect to the wording of independent references.
% % linguistic variations with respect to the wording of independent references.
% correct linguistic variations with respect to the wording of independent references, which are accounted for by post-editors.
% %correct but alternative wording  references.
% %correct but alternative formulations of the wording of independent references.
A key 
%ingredient
element of our multi-faceted analysis is human post-editing (PE), which consists in manually correcting systems' outputs according to the input (the source audio in our case). In PE-based evaluation, the original outputs are 
%then
compared against their post-edited version 
%(instead of independent references)
(rather than independent references) 
%to compute TER-based automatic metrics \cite{Snover:06}. 
through distance-based metrics like TER \cite{Snover:06}.
This allows 
%for 
counting only the true errors made by a system instead of penalising 
%also 
correct linguistic variations with respect to 
%the wording of independent references. 
references' wording.
%which are accounted for by post-editors.
This makes  PE-based evaluation one of the 
%most 
prominent  methodologies  used  for translation quality  assessment
%~\citep{Snover:06,Denkowski:2010,snover2009fluency,C16-1294,BentivogliIWSLT:2018}.
\citep{Snover:06,snover2009fluency,Denkowski:2010,Cettolo:2013,Bojar2015FindingsOT,C16-1294,BentivogliIWSLT:2018}.
%, which was chosen as  official evaluation in large-scale shared tasks, such as IWSLT from 2013 to 2017~\citep{Cettolo:2013} and the MT Quality Estimation Task at WMT-2015~\citep{Bojar2015FindingsOT}.
% This offers us a consolidated framework and best practices on which we can draw upon in our experiments. 
%
%
%The MuST-C \textit{Common} test set includes segments from talks that are common to all directions, thus making it possible to evaluate and compare systems across languages. 
 %The \textit{Common} test sets of the three directions addressed in this paper are composed of the same 27 TED talks, for a total of around 2,500 segments, and include one reference translation manually created from scratch. 
%
%
% For each language direction, we selected a subset of 550 segments -- henceforth \textit{PE-set} -- corresponding to about 10,000 English source words. To ensure the quality of the PE-set, we carried out a manual preparatory check and included only those segments i) containing speech and ii) for which  audio-transcript-translation alignment was correct. 
%
%For each language direction, we selected the same English audio portions from each talk, so to obtain representative groups of consecutive segments which are comparable across languages. Furthermore, to ensure the quality of the data, we carried out a manual preparatory check and included only those segments i) containing speech and ii) for which  audio-transcript-translation alignment was correct. The resulting test set -- henceforth \textit{PE-set} -- is composed of 550 segments, corresponding to about 10,000 English source words.
%
%%%%%%%%%%%%%%%%%%%%%%
% PROCEDURA SEGUITA
% Sentences were selected in a way to represent all the talks in the dataset proportionally to their length.  For each talk, three groups of consecutive sentences were selected from different parts of the talk: one close to the beginning, one in the middle, and one close to the end. The same selection criterion was applied to all the $11$ sections of MuST-C subject to manual evaluation, so to maximize the overlap between the sentences in the different languages and ensure results' comparability.
%%%%%%%%%%%%%%%%%%%%%%
%
%(around 90\%).
%
% For each language direction we selected a subset  of 550 segments -- henceforth \textit{PE-set} -- corresponding to about 10,000 English source words. These segments \textit{(i)} represent all the 27 common talks (groups of consecutive segments were extracted from different parts of each talk) and \textit{(ii)} were manually checked to ensure the correctness of the \textit{audio}-\textit{transcript}-\textit{translation} alignment, which in MuST-C is carried out automatically. 
%%Note that the PE-sets created for the three language pairs are not completely identical for two reasons: i) MuST-C talks are automatically segmented and  can thus result in different segments across languages; ii) we discarded all those segments for which  audio-transcript-translation alignment turned out to be incorrect (around 10\%). Although not exactly identical, the three PE-sets are largely overlapping.
%
The output of our cascade and direct systems run on the PE-sets was post-edited according to the  procedure adopted in the IWSLT PE-based evaluation campaigns \citep{Cettolo:2013}.
% Our cascade and direct systems 
% %(see $\S$\ref{ssec:systems}) 
% were  run on the PE-sets to be post-edited according to the experimental procedure adopted in the IWSLT PE-based evaluations campaigns \citep{Cettolo:2013}. 
To guarantee high quality post-edits, for each language we hired two professional translators with experience in  subtitling and post-editing. 
%%%%%AGGIUNTO PER RISPONDERE A MARCO
Furthermore, in order to cope with translators' variability 
%(i.e. 
%(one translator could systematically correct more than the other), 
the outputs of the two ST systems were randomly 
%assigned to them, 
assigned, ensuring that each translator worked on all the segments, %by 
equally post-editing both systems.
%
The post-editing task was performed with a 
%traditional CAT tool, which
CAT tool that displays the manual transcript of the audio together with the ST output to be edited. However, since ST systems take as input an audio signal, we also provided translators with the audio file of each segment, asking them to post-edit strictly according to it.\footnote{The \textit{ad-hoc} ST PE guidelines given to translators are included in the supplementary material.} 

%\paragraph{Additional analyses.}
\paragraph{Analyses.}
%
%The collected post-edits are exploited to assess overall systems' performance ($\S$\ref{sec:results}) as well as to carry out additional automatic analyses ($\S$\ref{sec:audio} and $\S$\ref{subsec:auto-errors}), aimed to shed light on possible systematic differences between the two paradigms. These analyses are complemented by fine-grained manual investigations ($\S$\ref{subsec:man-audio} and $\S$\ref{subsec:man-errors}) aimed to explore specific aspects in the behaviour of the systems. 
%These are done both manually and automatically, focusing on specific aspects (audio properties in $\S$\ref{sec:audio} and linguistic errors in $\S$\ref{sec:errors}) to shed light on possible systematic differences 
%between the two paradigms
%in systems' behaviour. These inspections are carried out by directly comparing the audio inputs with the systems' outputs, and do not require post-edits. Because of its linguistic nature, the annotation of the outputs was carried out by researchers with a strong background in linguistics and translation studies,  and excellent knowledge of both English and the target language (C2 or native).
%
%
The collected post-edits are exploited to assess overall systems' performance ($\S$\ref{sec:results}) as well as to carry out deeper quantitative and qualitative analyses
aimed to shed light on possible systematic differences in systems' behaviour ($\S$\ref{sec:audio}-\ref{sec:errors}). Focusing on 
%specific aspects (audio properties in $\S$\ref{sec:audio}, linguistic errors in $\S$\ref{sec:errors}),
specific aspects of the ST problem, the inquiry is performed  both automatically and by means of manual annotations.
Because of its linguistic nature, manual output annotations were carried out by researchers with a strong background in linguistics and translation studies,  and excellent knowledge of both English and the target language (C2 or native).



%%% ASCERTAINED PIECE
%Now that we have ascertained systems' parity in terms of overall performance, we delve into a number of different analyses -- both automatic and manual -- aimed to shed light on possible aspects peculiar to the different approaches. To this purpose, we focus on two main aspects: differences in performance due to specific input audio properties ($\S$\ref{sec:audio}) and with respect to linguistic errors ($\S$\ref{sec:errors}).
